Falcon2-11B Technical Report

We introduce Falcon2-11B, a foundation model trained on over five trillion tokens, and its multimodal counterpart, Falcon2-11B-vlm, which is a vision-to-text model. We report our findings during the training of the Falcon2-11B which follows a multi-stage approach where the early stages are distinguished by their context length and a final stage where we use a curated, high-quality dataset. Additionally, we report the effect of doubling the batch size mid-training and how training loss spikes are affected by the learning rate. The downstream performance of the foundation model is evaluated on established benchmarks, including multilingual and code datasets. The foundation model shows strong generalization across all the tasks which makes it suitable for downstream finetuning use cases. For the vision language model, we report the performance on several benchmarks and show that our model achieves a higher average score compared to open-source models of similar size. The model weights and code of both Falcon2-11B and Falcon2-11B-vlm are made available under a permissive license.

==> Falcon2_11B_Technical_Report/conversation_graph.tex <==
\GRAPH convosGraph

\begin{figure}[H]
\begin{center}



\begin{tikzpicture}[
dot/.style = {circle, fill, minimum size=#1,
                inner sep=0pt, outer sep=0pt},
               scale=0.45, every node/.style={scale=0.45}
]]
\draw[fill=fine-tuning] (0.0, -0.7) rectangle (1.4, 0.7);
\node at (0.7, 0.0) {\large  \phantom{lj}Do\phantom{lj}};
%%\node[below] at (0.7, 0.0) {\large  \phantom{lj}0\phantom{lj}};
\draw[fill=fine-tuning] (1.4, -0.7) rectangle (2.8, 0.7);
\node at (2.0999999999999996, 0.0) {\large  \phantom{lj}you\phantom{lj}};
%\node[below] at (2.0999999999999996, 0.0) {\large  \phantom{lj}1\phantom{lj}};
\draw[fill=fine-tuning] (2.8000000000000003, -0.7) rectangle (4.2, 0.7);
\node at (3.5, 0.0) {\large  \phantom{lj}like\phantom{lj}};
%\node[below] at (3.5, 0.0) {\large  \phantom{lj}2\phantom{lj}};
\draw[fill=fine-tuning] (4.200000000000001, -0.7) rectangle (5.6000000000000005, 0.7);
\node at (4.9, 0.0) {\large  \phantom{lj}Venice?\phantom{lj}};
%\node[below] at (4.9, 0.0) {\large  \phantom{lj}3\phantom{lj}};
\draw[fill=objective] (6.4, 0.10000000000000009) rectangle (7.800000000000001, 1.5);
\node at (7.1000000000000005, 0.8) {\large  \phantom{lj}Not\phantom{lj}};
%\node[below] at (7.1000000000000005, 0.8) {\large  \phantom{lj}4\phantom{lj}};
\draw[fill=objective] (7.800000000000001, 0.10000000000000009) rectangle (9.200000000000001, 1.5);
\node at (8.5, 0.8) {\large  \phantom{lj}really,\phantom{lj}};
%\node[below] at (8.5, 0.8) {\large  \phantom{lj}5\phantom{lj}};
\draw[fill=objective] (9.200000000000003, 0.10000000000000009) rectangle (10.600000000000003, 1.5);
\node at (9.900000000000002, 0.8) {\large  \phantom{lj}it's\phantom{lj}};
%\node[below] at (9.900000000000002, 0.8) {\large  \phantom{lj}6\phantom{lj}};
\draw[fill=objective] (10.600000000000005, 0.10000000000000009) rectangle (12.000000000000005, 1.5);
\node at (11.300000000000004, 0.8) {\large  \phantom{lj}always\phantom{lj}};
%\node[below] at (11.300000000000004, 0.8) {\large  \phantom{lj}7\phantom{lj}};
\draw[fill=objective] (12.000000000000007, 0.10000000000000009) rectangle (13.550000000000007, 1.5);
\node at (12.750000000000006, 0.8) {\large  \phantom{lj}flooded\phantom{lj}};
%\node[below] at (12.700000000000006, 0.8) {\large  \phantom{lj}8\phantom{lj}};
\draw[fill=architecture] (14.200000000000008, 0.9000000000000001) rectangle (15.600000000000009, 2.3);
\node at (14.90000000000001, 1.6) {\large  \phantom{lj}Oh,\phantom{lj}};
%\node[below] at (14.90000000000001, 1.6) {\large  \phantom{lj}9\phantom{lj}};
\draw[fill=architecture] (15.600000000000007, 0.9000000000000001) rectangle (17.000000000000007, 2.3);
\node at (16.300000000000008, 1.6) {\large  \phantom{lj}I\phantom{lj}};
%\node[below] at (16.300000000000008, 1.6) {\large  \phantom{lj}10\phantom{lj}};
\draw[fill=architecture] (17.000000000000007, 0.9000000000000001) rectangle (18.400000000000006, 2.3);
\node at (17.700000000000006, 1.6) {\large  \phantom{lj}agree\phantom{lj}};
%\node[below] at (17.700000000000006, 1.6) {\large  \phantom{lj}11\phantom{lj}};
\draw[fill=evaluation] (14.200000000000008, -0.7) rectangle (15.600000000000009, 0.7);
\node at (14.90000000000001, 0.0) {\large  \phantom{lj}Really?\phantom{lj}};
%\node[below] at (14.90000000000001, 0.0) {\large  \phantom{lj}9\phantom{lj}};
\draw[fill=evaluation] (15.600000000000007, -0.7) rectangle (17.000000000000007, 0.7);
\node at (16.300000000000008, 0.0) {\large  \phantom{lj}it's\phantom{lj}};
%\node[below] at (16.300000000000008, 0.0) {\large  \phantom{lj}10\phantom{lj}};
\draw[fill=evaluation] (17.000000000000007, -0.7) rectangle (18.400000000000006, 0.7);
\node at (17.700000000000006, 0.0) {\large  \phantom{lj}so\phantom{lj}};
%\node[below] at (17.700000000000006, 0.0) {\large  \phantom{lj}11\phantom{lj}};
\draw[fill=evaluation] (18.400000000000006, -0.7) rectangle (19.800000000000004, 0.7);
\node at (19.100000000000005, 0.0) {\large  \phantom{lj}nice!\phantom{lj}};
%\node[below] at (19.100000000000005, 0.0) {\large  \phantom{lj}12\phantom{lj}};
\draw[fill=adaptation] (6.4, -1.5) rectangle (7.800000000000001, -0.10000000000000009);
\node at (7.1000000000000005, -0.8) {\large  \phantom{lj}Yes!\phantom{lj}};
%\node[below] at (7.1000000000000005, -0.8) {\large  \phantom{lj}4\phantom{lj}};
\draw[fill=adaptation] (7.800000000000001, -1.5) rectangle (9.200000000000001, -0.10000000000000009);
\node at (8.5, -0.8) {\large  \phantom{lj}It's\phantom{lj}};
%\node[below] at (8.5, -0.8) {\large  \phantom{lj}5\phantom{lj}};
\draw[fill=adaptation] (9.200000000000003, -1.5) rectangle (10.600000000000003, -0.10000000000000009);
\node at (9.900000000000002, -0.8) {\large  \phantom{lj}unique!\phantom{lj}};
%\node[below] at (9.900000000000002, -0.8) {\large  \phantom{lj}6\phantom{lj}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5



% \draw[pattern=north west lines, pattern color=fine-tuning] (0.0, -4.7) rectangle (1.4, -3.3000000000000003);
\draw[fill=fine-tuning] (0.0, -4.7) rectangle (1.4, -3.3000000000000003);
\node at (0.7, -4.0) {\large  \phantom{lj}Do\phantom{lj}};
%\node[below] at (0.7, -4.0) {\large  \phantom{lj}0\phantom{lj}};
% \draw[pattern=north west lines, pattern color=fine-tuning] (1.4, -4.7) rectangle (2.8, -3.3000000000000003);
\draw[fill=fine-tuning] (1.4, -4.7) rectangle (2.8, -3.3000000000000003);
\node at (2.0999999999999996, -4.0) {\large  \phantom{lj}you\phantom{lj}};
%\node[below] at (2.0999999999999996, -4.0) {\large  \phantom{lj}1\phantom{lj}};
% \draw[pattern=north west lines, pattern color=fine-tuning] (2.8000000000000003, -4.7) rectangle (4.2, -3.3000000000000003);
\draw[fill=fine-tuning] (2.8000000000000003, -4.7) rectangle (4.2, -3.3000000000000003);
\node at (3.5, -4.0) {\large  \phantom{lj}like\phantom{lj}};
%\node[below] at (3.5, -4.0) {\large  \phantom{lj}2\phantom{lj}};
% \draw[pattern=north west lines, pattern color=fine-tuning] (4.200000000000001, -4.7) rectangle (5.6000000000000005, -3.3000000000000003);
\draw[fill=fine-tuning] (4.200000000000001, -4.7) rectangle (5.6000000000000005, -3.3000000000000003);
\node at (4.9, -4.0) {\large  \phantom{lj}Venice?\phantom{lj}};
%\node[below] at (4.9, -4.0) {\large  \phantom{lj}3\phantom{lj}};
% \draw[pattern=north west lines, pattern color=objective] (5.6000000000000005, -4.7) rectangle (7.0, -3.3000000000000003);
\draw[fill=objective] (5.6000000000000005, -4.7) rectangle (7.0, -3.3000000000000003);
\node at (6.300000000000001, -4.0) {\large  \phantom{lj}Not\phantom{lj}};
%\node[below] at (6.300000000000001, -4.0) {\large  \phantom{lj}4\phantom{lj}};
% \draw[pattern=north west lines, pattern color=objective] (6.999999999999999, -4.7) rectangle (8.399999999999999, -3.3000000000000003);
\draw[fill=objective] (6.999999999999999, -4.7) rectangle (8.399999999999999, -3.3000000000000003);
\node at (7.699999999999999, -4.0) {\large  \phantom{lj}really,\phantom{lj}};
%\node[below] at (7.699999999999999, -4.0) {\large  \phantom{lj}5\phantom{lj}};
% \draw[pattern=north west lines, pattern color=objective] (8.399999999999999, -4.7) rectangle (9.799999999999997, -3.3000000000000003);
\draw[fill=objective] (8.399999999999999, -4.7) rectangle (9.799999999999997, -3.3000000000000003);
\node at (9.099999999999998, -4.0) {\large  \phantom{lj}it's\phantom{lj}};
%\node[below] at (9.099999999999998, -4.0) {\large  \phantom{lj}6\phantom{lj}};
% \draw[pattern=north west lines, pattern color=objective] (9.799999999999997, -4.7) rectangle (11.199999999999996, -3.3000000000000003);
\draw[fill=objective] (9.799999999999997, -4.7) rectangle (11.199999999999996, -3.3000000000000003);
\node at (10.499999999999996, -4.0) {\large  \phantom{lj}always\phantom{lj}};
%\node[below] at (10.499999999999996, -4.0) {\large  \phantom{lj}7\phantom{lj}};
% \draw[pattern=north west lines, pattern color=objective] (11.199999999999996, -4.7) rectangle (12.749999999999994, -3.3000000000000003);
\draw[fill=objective] (11.199999999999996, -4.7) rectangle (12.749999999999994, -3.3000000000000003);
\node at (11.949999999999995, -4.0) {\large  \phantom{lj}flooded\phantom{lj}};
%\node[below] at (11.899999999999995, -4.0) {\large  \phantom{lj}8\phantom{lj}};
\draw[fill=architecture] (12.749999999999994, -4.7) rectangle (13.999999999999995, -3.3000000000000003);
\node at (13.299999999999994, -4.0) {\large  \phantom{lj}Oh,\phantom{lj}};
%\node[below] at (13.299999999999994, -4.0) {\large  \phantom{lj}9\phantom{lj}};
\draw[fill=architecture] (13.999999999999996, -4.7) rectangle (15.399999999999997, -3.3000000000000003);
\node at (14.699999999999996, -4.0) {\large  \phantom{lj}I\phantom{lj}};
%\node[below] at (14.699999999999996, -4.0) {\large  \phantom{lj}10\phantom{lj}};
\draw[fill=architecture] (15.399999999999999, -4.7) rectangle (16.799999999999997, -3.3000000000000003);
\node at (16.099999999999998, -4.0) {\large  \phantom{lj}agree\phantom{lj}};
%\node[below] at (16.099999999999998, -16.0) {\large  \phantom{lj}11\phantom{lj}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[pattern=north west lines, pattern color=fine-tuning] (0.0, -6.7) rectangle (1.4, -5.3000000000000003);
\node at (0.7, -6.0) {\large  \phantom{lj}Do\phantom{lj}};
%\node[below] at (0.7, -6.0) {\large  \phantom{lj}0\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (1.4, -6.7) rectangle (2.8, -5.3000000000000003);
\node at (2.0999999999999996, -6.0) {\large  \phantom{lj}you\phantom{lj}};
%\node[below] at (2.0999999999999996, -6.0) {\large  \phantom{lj}1\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (2.8000000000000003, -6.7) rectangle (4.2, -5.3000000000000003);
\node at (3.5, -6.0) {\large  \phantom{lj}like\phantom{lj}};
%\node[below] at (3.5, -6.0) {\large  \phantom{lj}2\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (4.200000000000001, -6.7) rectangle (5.6000000000000005, -5.3000000000000003);
\node at (4.9, -6.0) {\large  \phantom{lj}Venice?\phantom{lj}};
%\node[below] at (4.9, -6.0) {\large  \phantom{lj}3\phantom{lj}};
\draw[pattern=north west lines, pattern color=objective] (5.6000000000000005, -6.7) rectangle (7.0, -5.3000000000000003);
\node at (6.300000000000001, -6.0) {\large  \phantom{lj}Not\phantom{lj}};
%\node[below] at (6.300000000000001, -6.0) {\large  \phantom{lj}4\phantom{lj}};
\draw[pattern=north west lines, pattern color=objective] (6.999999999999999, -6.7) rectangle (8.399999999999999, -5.3000000000000003);
\node at (7.699999999999999, -6.0) {\large  \phantom{lj}really,\phantom{lj}};
%\node[below] at (7.699999999999999, -6.0) {\large  \phantom{lj}5\phantom{lj}};
\draw[pattern=north west lines, pattern color=objective] (8.399999999999999, -6.7) rectangle (9.799999999999997, -5.3000000000000003);
\node at (9.099999999999998, -6.0) {\large  \phantom{lj}it's\phantom{lj}};
%\node[below] at (9.099999999999998, -6.0) {\large  \phantom{lj}6\phantom{lj}};
\draw[pattern=north west lines, pattern color=objective] (9.799999999999997, -6.7) rectangle (11.199999999999996, -5.3000000000000003);
\node at (10.499999999999996, -6.0) {\large  \phantom{lj}always\phantom{lj}};
%\node[below] at (10.499999999999996, -6.0) {\large  \phantom{lj}7\phantom{lj}};
\draw[pattern=north west lines, pattern color=objective] (11.199999999999996, -6.7) rectangle (12.749999999999994, -5.3000000000000003);
\node at (11.949999999999995, -6.0) {\large  \phantom{lj}flooded\phantom{lj}};
%\node[below] at (11.899999999999995, -6.0) {\large  \phantom{lj}8\phantom{lj}};
\draw[fill=evaluation] (12.749999999999994, -6.7) rectangle (14.099999999999995, -5.3000000000000003);
\node at (13.399999999999994, -6.0) {\large  \phantom{lj}Really?\phantom{lj}};
%\node[below] at (13.299999999999994, -6.0) {\large  \phantom{lj}9\phantom{lj}};
\draw[fill=evaluation] (14.099999999999995, -6.7) rectangle (15.399999999999997, -5.3000000000000003);
\node at (14.699999999999996, -6.0) {\large  \phantom{lj}it's\phantom{lj}};
%\node[below] at (14.699999999999996, -6.0) {\large  \phantom{lj}10\phantom{lj}};
\draw[fill=evaluation] (15.399999999999999, -6.7) rectangle (16.799999999999997, -5.3000000000000003);
\node at (16.099999999999998, -6.0) {\large  \phantom{lj}so\phantom{lj}};
%\node[below] at (16.099999999999998, -6.0) {\large  \phantom{lj}11\phantom{lj}};
\draw[fill=evaluation] (16.799999999999997, -6.7) rectangle (18.199999999999996, -5.3000000000000003);
\node at (17.499999999999996, -6.0) {\large  \phantom{lj}nice!\phantom{lj}};
%\node[below] at (17.499999999999996, -6.0) {\large  \phantom{lj}9\phantom{lj}};



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\draw[pattern=north west lines, pattern color=fine-tuning] (0.0, -8.7) rectangle (1.4, -7.3000000000000003);
\node at (0.7, -8.0) {\large  \phantom{lj}Do\phantom{lj}};
%\node[below] at (0.7, -8.0) {\large  \phantom{lj}0\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (1.4, -8.7) rectangle (2.8, -7.3000000000000003);
\node at (2.0999999999999996, -8.0) {\large  \phantom{lj}you\phantom{lj}};
%\node[below] at (2.0999999999999996, -8.0) {\large  \phantom{lj}1\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (2.8000000000000003, -8.7) rectangle (4.2, -7.3000000000000003);
\node at (3.5, -8.0) {\large  \phantom{lj}like\phantom{lj}};
%\node[below] at (3.5, -8.0) {\large  \phantom{lj}2\phantom{lj}};
\draw[pattern=north west lines, pattern color=fine-tuning] (4.200000000000001, -8.7) rectangle (5.6000000000000005, -7.3000000000000003);
\node at (4.9, -8.0) {\large  \phantom{lj}Venice?\phantom{lj}};
%\node[below] at (4.9, -8.0) {\large  \phantom{lj}3\phantom{lj}};
\draw[fill=adaptation] (5.6000000000000005, -8.7) rectangle (7.0, -7.3000000000000003);
\node at (6.300000000000001, -8.0) {\large  \phantom{lj}Yes!\phantom{lj}};
%\node[below] at (6.300000000000001, -8.0) {\large  \phantom{lj}4\phantom{lj}};
\draw[fill=adaptation] (6.999999999999999, -8.7) rectangle (8.399999999999999, -7.3000000000000003);
\node at (7.699999999999999, -8.0) {\large  \phantom{lj}It's\phantom{lj}};
%\node[below] at (7.699999999999999, -8.0) {\large  \phantom{lj}5\phantom{lj}};
\draw[fill=adaptation] (8.399999999999999, -8.7) rectangle (9.799999999999997, -7.3000000000000003);
\node at (9.099999999999998, -8.0) {\large  \phantom{lj}unique!\phantom{lj}};
%\node[below] at (9.099999999999998, -8.0) {\large  \phantom{lj}6\phantom{lj}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[pattern=north west lines, pattern color=black] (19.049999999999994, -4.25) rectangle (19.549999999999994, -3.75);
\node[right] at (19.549999999999994, -4) {\Large Loss masked};
% \draw[fill=black] (19.049999999999994, -4.7) rectangle (19.549999999999994, -4.2);
% \node[right] at (19.549999999999994, -4.45) {\Large Not Masked};


%(15.399999999999999, -12.7) rectangle (16.799999999999997, -11.3000000000000003)






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \draw[-{Latex[width=1.5mm]},] (5.6000000000000005, 0.0) to [bend left = 0] (6.4, 0.8);
% \draw[-{Latex[width=1.5mm]},] (13.550000000000007, 0.8) to [bend left = 0] (14.200000000000008, 1.6);
% \draw[-{Latex[width=1.5mm]},] (13.550000000000007, 0.8) to [bend left = 0] (14.200000000000008, 0.0);
% \draw[-{Latex[width=1.5mm]},] (5.6000000000000005, 0.0) to [bend left = 0] (6.4, -0.8);

\draw[->,] (5.6000000000000005, 0.0) to [bend left = 0] (6.4, 0.8);
\draw[->,] (13.550000000000007, 0.8) to [bend left = 0] (14.200000000000008, 1.6);
\draw[->,] (13.550000000000007, 0.8) to [bend left = 0] (14.200000000000008, 0.0);
\draw[->,] (5.6000000000000005, 0.0) to [bend left = 0] (6.4, -0.8);


\end{tikzpicture}
\captionof{figure}{Visualization of conversation tree flattening and loss masking. In this simple example, the token count of the conversation tree is 19, while the flattened conversation tree contains the 19 initial tokens, but also contains 13 repeated tokens with masked loss, producing an overhead of $+68\%$.} 
\label{fig:convosGraph}


\end{center}
\end{figure}


\ENDGRAPH

==> Falcon2_11B_Technical_Report/figure_vlm.tex <==
\begin{figure}[H]
\begin{center}


\resizebox{\textwidth}{!}{
\begin{tikzpicture}[line width=2]
    \def\gridWidth{14}
    \def\gridCenter{8}
    \def\gridHeight{6}
    \def\rectWidth{0.8}
    \def\rectHeight{0.8}
    \def\spacing{0.2}
    \def\halfImages{3}
    \pgfmathsetmacro{\thresholdImages}{2*\halfImages + 1}
    \pgfmathsetmacro{\tokenDots}{\halfImages + 1}
    \def\braceHeight{1}
    \def\arrowHeight{0.8}
    \def\imageSide{5}
    \def\patchSide{0.8}
    \def\patchSidecm{0.8cm}
    \def\nGeneratedTokens{7}
    \pgfmathsetmacro{\xDots}{\tokenDots + 0.5*\rectWidth}
    \pgfmathsetmacro{\yDots}{0.5*\rectHeight}
    \pgfmathsetmacro{\yFalcon}{\spacing + \rectHeight}
    \pgfmathsetmacro{\falconWidth}{\gridWidth - \spacing + \nGeneratedTokens - 1}
    \pgfmathsetmacro{\totalTokens}{\gridWidth + \nGeneratedTokens - 1}
    \pgfmathsetmacro{\yProjector}{-\rectHeight - \arrowHeight} % -\braceHeight
    \pgfmathsetmacro{\yTokens}{\yProjector - \rectHeight - \spacing}
    \pgfmathsetmacro{\yVisionEncoder}{\yProjector - \arrowHeight - \rectHeight - \rectHeight - \spacing}
    \pgfmathsetmacro{\projectorWidth}{\thresholdImages-\spacing}
    \pgfmathsetmacro{\tokenizerWidth}{\gridWidth - \thresholdImages - \spacing}
    \pgfmathsetmacro{\embWidth}{\tokenizerWidth + \nGeneratedTokens - 1}

    \pgfmathsetmacro{\xTokenizer}{\thresholdImages-\spacing}
    \pgfmathsetmacro{\yPatches}{\yVisionEncoder-\spacing-0.5*\patchSide}
    \pgfmathsetmacro{\yImage}{\yPatches - 0.5*\imageSide -0.5*\patchSide - \arrowHeight}    
    \foreach \x in {1,2,...,\gridWidth} {
            \ifnum \x > \thresholdImages
                \def\colorToken{blue!20}
            \else
                \def\colorToken{red!20}
            \fi
            \ifnum \x = \tokenDots
                \node at (\xDots, \yDots) {\dots};
            \else
                \draw[fill=\colorToken] (\x,0) rectangle ++(\rectWidth, \rectHeight);
            \fi
    }
    % falcon box
    \draw[fill=green!20] (1, \yFalcon) rectangle ++(\falconWidth, \rectHeight);
    \node at (1 + 0.5*\falconWidth, \yFalcon + 0.5*\rectHeight) {\Large Falcon2-11B LLM (Chat Finetuned) $f_{LLM}(\cdot)$};

    % projector box
    \draw[fill=red!20] (1, \yProjector) rectangle ++(\projectorWidth, \rectHeight);
    \node at (1 + 0.5*\projectorWidth, \yProjector + 0.5*\rectHeight) {\Large Projector $f_{proj}(\cdot)$};

    % arrow vision projector -> tokens
    \draw[->] (1 + 0.5*\projectorWidth,\yProjector+\rectHeight) -- (1 + 0.5*\projectorWidth,0) node[midway, right] {\Large $\bm{H}_p$};

    % vision encoder box
    \draw[fill=red!20] (1, \yVisionEncoder) rectangle ++(\projectorWidth, \rectHeight);
    \node at (1 + 0.5*\projectorWidth, \yVisionEncoder + 0.5*\rectHeight) {\Large Vision Encoder $f_e(\cdot)$};    

    % arrow vision encoder -> projector
    \draw[->] (1 + 0.5*\projectorWidth,\yVisionEncoder+\rectHeight) -- (1 + 0.5*\projectorWidth,\yProjector) node[midway, right] {\Large $\bm{H}_e$};

    % image patches
    \foreach \x in {1,2,...,\halfImages} {
        \ifnum \x = 1
            \node at (\x + 0.5*\patchSide, \yPatches) {\includegraphics[width=\patchSide cm, height=\patchSide cm,trim=0cm 11.25cm 11.25cm 0cm, clip]{figures/cropped_falcon.jpg}};
            \node at (\x + 0.5*\patchSide + \halfImages + 1, \yPatches) {\includegraphics[width=\patchSidecm, height=\patchSide cm,trim=8.75cm 0cm 2.5cm 11.25cm, clip]{figures/cropped_falcon.jpg}}; 
        \fi
        \ifnum \x = 2
            \node at (\x + 0.5*\patchSide, \yPatches) {\includegraphics[width=\patchSide cm, height=\patchSide cm,trim=1.25cm 11.25cm 10cm 0cm, clip]{figures/cropped_falcon.jpg}};
            \node at (\x + 0.5*\patchSide + \halfImages + 1, \yPatches) {\includegraphics[width=\patchSidecm, height=\patchSide cm,trim=10cm 0cm 1.25cm 11.25cm, clip]{figures/cropped_falcon.jpg}};        
        \fi
        \ifnum \x = 3
            \node at (\x + 0.5*\patchSide, \yPatches) {\includegraphics[width=\patchSide cm, height=\patchSide cm,trim=2.5cm 11.25cm 8.75cm 0cm, clip]{figures/cropped_falcon.jpg}};
            \node at (\x + 0.5*\patchSide + \halfImages + 1, \yPatches) {\includegraphics[width=\patchSidecm, height=\patchSide cm,trim=11.25cm 0cm 0cm 11.25cm, clip]{figures/cropped_falcon.jpg}};
        \fi
    }
    % dots in patches
    \node at (\xDots, \yPatches) {\dots};
    
    %image
    \node at (1 + 0.5*\projectorWidth, \yImage) {\includegraphics[width=\imageSide cm, height=\imageSide cm]{figures/cropped_falcon.jpg}};

    % arrow image -> patches
    \draw[->] (1 + 0.5*\projectorWidth,\yImage+0.5*\imageSide) -- (1 + 0.5*\projectorWidth,\yPatches-0.5*\patchSide);


    % embedding box
    \draw[fill=blue!20] (1 + \projectorWidth + \spacing, \yProjector) rectangle ++(\embWidth, \rectHeight);
    \node at (1 + \projectorWidth + \spacing + 0.5*\embWidth, \yProjector + 0.5*\rectHeight) {\Large Embedding};

    % arrow embedding -> tokens
    \draw[->] (1 + \projectorWidth + \spacing + 0.5*\embWidth,\yProjector+\rectHeight) -- (1 + \projectorWidth + \spacing + 0.5*\embWidth,0) node[midway, right] {\Large $\bm{H}_t$};

    % vision encoder box
    \draw[fill=blue!20] (1 + \projectorWidth + \spacing, \yVisionEncoder) rectangle ++(\tokenizerWidth, \rectHeight);
    \node at (1 + \projectorWidth + \spacing + 0.5*\tokenizerWidth, \yVisionEncoder + 0.5*\rectHeight) {\Large Tokenizer};

    % text
    \node at (1 + \projectorWidth + \spacing + 0.5*\tokenizerWidth, \yPatches) {\large  \textit{User: What species is this bird? Falcon:}};

    % generated token
    \def\generatedTokensList{{The}, {bird}, {is}, {a}, {falcon}, {.},{\textbf{eos}}}
    \foreach \str [count=\x from \gridWidth] in \generatedTokensList {
        \ifnum \x = \gridWidth
            \draw[fill=gray!30] (\x,2*\spacing+2*\rectHeight) rectangle ++(\rectWidth, \rectHeight) node[pos=0.5] {\tiny \str} node[midway, left=4mm] {generated tokens};
        \else
            \ifnum \x > \totalTokens
            \else
                \draw[fill=gray!30] (\x,2*\spacing+2*\rectHeight) rectangle ++(\rectWidth, \rectHeight) node[pos=0.5] {\tiny \str};
            \fi
        \fi
    }
    % generated tokens in embedding
    \foreach \str [count=\x from \gridWidth] in \generatedTokensList {
    \ifnum \x < \totalTokens
        \pgfmathsetmacro{\actx}{\x+1}
        \draw[fill=gray!30] (\actx,\yTokens) rectangle ++(\rectWidth, \rectHeight) node[pos=0.5] {\tiny \str};
        \draw[fill=gray!30] (\actx,0) rectangle ++(\rectWidth, \rectHeight);
        \fi
    }

    % input tokens
    \def\myList{{User:}, {What}, {spieces}, {is}, {this}, {bird} {?},{Falcon:}, {dummy}}
    \pgfmathsetmacro{\start}{\thresholdImages + 1}
    \foreach \str [count=\x from \start] in \myList {
        \ifnum \x > \gridWidth
        \else
            \draw[fill=blue!20] (\x,\yTokens) rectangle ++(\rectWidth, \rectHeight) node[pos=0.5] {\tiny \str};
        \fi
    }

    % arrow tokenizer -> tokens
    \draw[->] (1 + \projectorWidth + \spacing + 0.5*\tokenizerWidth,\yVisionEncoder+\rectHeight) -- (1 + \projectorWidth + \spacing + 0.5*\tokenizerWidth,\yTokens);
\end{tikzpicture}
}



\caption{Falcon2-11B VLM architecture. See \cref{falcon_vlm} for details.} 
\label{fig:vlm}


\end{center}
\end{figure}
